M2K: II. A Triple-Planet System Orbiting HIP 57274

Doppler observations from Keck Observatory have revealed a triple planet system orbiting the nearby mid-type K dwarf, HIP 57274. The inner planet, HIP 57274b, is a super-Earth with \msini\ = 11.6 \mearth (0.036 \mjup), an orbital period of 8.135 $\pm$ 0.004 d, and slightly eccentric orbit $e=0.19 \pm 0.1$. We calculate a transit probability of 6.5% for the inner planet. The second planet has \msini\ = 0.4 \mjup\ with an orbital period of 32.0 $\pm 0.02$ d in a nearly circular orbit, and $e = 0.05 \pm 0.03$. The third planet has \msini\ = 0.53 \mjup\ with an orbital period of 432 $\pm 8$ d (1.18 years) and an eccentricity $e = 0.23 \pm 0.03$. This discovery adds to the number of super Earth mass planets with $\msini < 12 \mearth\ $ that have been detected with Doppler surveys. We find that 56 $\pm 18$% super-Earths are members of multi-planet systems. This is certainly a lower limit because of observational detectability limits, yet significantly higher than the fraction of Jupiter mass exoplanets, $20 \pm 8$%, that are members of Doppler-detected, multi-planet systems.

==> rv_table.tex <==
\begin{deluxetable}{rrccc}
\tablenum{2}
\tablecaption{Radial Velocities for HIP~57274}
\tablewidth{0pt}
\tablehead{ 
    \colhead{}   &
    \colhead{RV} & 
    \colhead{$\sigma_{\rm RV}$} &
    \colhead{$S_{HK}$}  \\
       \colhead{JD-2440000} & 
       \colhead{(\ms)} & 
       \colhead{(\ms)} & 
                       \\
 }
\startdata
    14806.13297  &     0.65  &     1.34  &     0.469  \\
    14807.14718  &    -2.97  &     1.88  &     0.469  \\
    14809.15850  &    -1.80  &     1.26  &     0.468  \\
    15190.15800  &   -14.89  &     1.18  &     0.409  \\
    15198.16272  &    -7.39  &     1.29  &     0.403  \\
    15232.04776  &    11.50  &     1.26  &     0.411  \\
    15255.86086  &    -7.77  &     1.12  &     0.417  \\
    15255.96257  &    -7.31  &     1.28  &     0.415  \\
    15260.92225  &    -5.73  &     1.32  &     0.411  \\
    15284.83929  &    -7.20  &     1.32  &     0.403  \\
    15285.97628  &    -7.78  &     1.57  &     0.393  \\
    15289.99940  &   -19.10  &     1.15  &     0.372  \\
    15312.86902  &    19.47  &     1.17  &     0.404  \\
    15313.94053  &     8.04  &     1.14  &     0.406  \\
    15314.78643  &     0.61  &     1.34  &     0.406  \\
    15317.97039  &   -12.74  &     1.16  &     0.419  \\
    15318.95571  &    -8.96  &     1.24  &     0.421  \\
    15320.91370  &    -8.58  &     1.17  &     0.424  \\
    15321.81404  &   -19.89  &     1.16  &     0.424  \\
    15342.88784  &    29.21  &     1.20  &     0.365  \\
    15343.85339  &    27.14  &     1.20  &     0.369  \\
    15344.87342  &    20.66  &     1.31  &     0.371  \\
    15350.86226  &   -10.80  &     1.13  &     0.395  \\
    15351.92024  &   -11.83  &     1.17  &     0.401  \\
    15372.80778  &    31.25  &     1.24  &     0.401  \\
    15375.78096  &    21.18  &     1.22  &     0.387  \\
    15377.74610  &     8.16  &     1.17  &     0.380  \\
    15379.79676  &   -15.79  &     1.31  &     0.371  \\
    15380.74874  &   -17.47  &     1.08  &     0.369  \\
    15395.82890  &    25.02  &     1.44  &     0.415  \\
    15396.82085  &    29.01  &     1.30  &     0.420  \\
    15399.81103  &    45.46  &     1.35  &     0.385  \\
    15400.75673  &    51.94  &     1.51  &     0.396  \\
    15403.75099  &    32.68  &     1.24  &     0.396  \\
    15404.75039  &    29.88  &     1.16  &     0.404  \\
    15405.74739  &    23.35  &     1.23  &     0.402  \\
    15406.74250  &    18.96  &     1.08  &     0.403  \\
    15407.76442  &    17.17  &     1.24  &     0.397  \\
    15410.74392  &     0.78  &     1.19  &     0.395  \\
    15411.73974  &    -9.68  &     1.31  &     0.392  \\
    15412.73624  &   -12.77  &     1.25  &     0.392  \\
    15413.74320  &   -21.86  &     1.24  &     0.388  \\
    15425.73431  &     6.04  &     1.37  &     0.370  \\
    15426.73083  &    10.65  &     1.24  &     0.377  \\
    15427.73759  &    13.29  &     1.30  &     0.377  \\
    15428.72751  &    16.56  &     1.33  &     0.368  \\
    15522.12170  &   -18.28  &     1.15  &     0.391  \\
    15529.16410  &    10.24  &     1.12  &     0.390  \\
    15543.14293  &   -59.09  &     1.17  &     0.378  \\
    15546.14908  &   -58.26  &     1.19  &     0.388  \\
    15557.04557  &     4.30  &     1.25  &     0.394  \\
    15559.13567  &     4.32  &     1.44  &     0.376  \\
    15585.10572  &   -15.50  &     1.16  &     0.399  \\
    15606.06452  &   -34.39  &     1.28  &     0.401  \\
    15607.09612  &   -40.58  &     1.19  &     0.399  \\
    15608.09774  &   -44.48  &     1.23  &     0.394  \\
    15614.08347  &   -25.65  &     1.27  &     0.383  \\
    15633.97134  &   -11.63  &     1.24  &     0.390  \\
    15635.08252  &   -13.77  &     1.42  &     0.393  \\
    15636.01755  &   -15.87  &     1.13  &     0.400  \\
    15636.92708  &   -18.25  &     1.24  &     0.397  \\
    15663.94826  &    12.71  &     1.20  &     0.377  \\
    15668.91659  &   -13.02  &     1.22  &     0.399  \\
    15670.84399  &   -17.81  &     1.13  &     0.405  \\
    15670.95361  &   -19.64  &     1.05  &     0.404  \\
    15671.82896  &   -23.09  &     1.09  &     0.406  \\
    15672.81592  &   -27.88  &     1.06  &     0.409  \\
    15673.82281  &   -24.19  &     1.13  &     0.406  \\
    15696.86668  &     2.84  &     1.27  &     0.379  \\
    15697.80266  &    -7.08  &     1.15  &     0.377  \\
    15698.80643  &    -8.48  &     1.24  &     0.374  \\
    15699.81078  &   -14.82  &     1.11  &     0.373  \\
    15700.82014  &   -16.82  &     1.12  &     0.372  \\
    15703.77349  &   -18.66  &     1.04  &     0.368  \\
    15704.75548  &   -30.18  &     1.16  &     0.365  \\
    15705.75509  &   -29.81  &     1.01  &     0.368  \\
    15706.79029  &   -28.32  &     1.21  &     0.369  \\
    15707.80564  &   -21.78  &     1.14  &     0.365  \\
    15723.77583  &    30.74  &     1.12  &     0.385  \\
    15728.75995  &     9.96  &     1.15  &     0.399  \\
    15733.76451  &   -11.87  &     1.18  &     0.392  \\
    15734.78802  &   -15.04  &     0.97  &     0.394  \\
    15735.76864  &   -19.76  &     1.11  &     0.396  \\
    15738.75911  &   -32.60  &     1.19  &     0.388  \\
    15751.75202  &    36.45  &     1.18  &     0.363  \\
    15752.74589  &    32.55  &     1.17  &     0.362  \\
    15759.75211  &    19.12  &     1.28  &     0.365  \\
    15760.74400  &    11.38  &     1.17  &     0.366  \\
    15761.74876  &    -0.77  &     1.21  &     0.369  \\
    15762.76237  &    -8.06  &     1.28  &     0.369  \\
    15763.75501  &   -13.88  &     1.21  &     0.368  \\
    15768.74088  &   -20.24  &     1.16  &     0.371  \\
    15770.75597  &   -30.11  &     1.36  &     0.369  \\
    15781.73264  &    30.82  &     1.31  &     0.382  \\
    15787.72792  &    30.85  &     1.38  &     0.377  \\
    15788.72674  &    26.29  &     1.36  &     0.369  \\
    15790.72301  &    17.15  &     1.38  &     0.342  \\
    15791.72929  &    19.16  &     1.15  &     0.368  \\
    15792.72765  &    12.17  &     1.23  &     0.367  \\
\enddata
\end{deluxetable}
\clearpage

